Spatial Consistency Evaluation Based on Massive SIMO Measurements

In this paper, the spatial consistency of wireless massive single-input-multiple-output channels in a cellular small cell scenario is evaluated based on measurements taken in Berlin city. The evaluation is done by computing the similarity of covariance matrices over the distance. As similarity measure the correlation matrix distance is used. A classification of the measurements tracks based on the shape of the curves into four different categories is done. The results in this paper indicate that spatial consistency is a highly deterministic property in the sense that it depends strongly on the individual environment and not so much on large scale parameters. Therefore, we conclude that spatial consistency is not sufficiently modelled by the current 3rd Generation Partnership Project feature.

==> header_paper.tex <==
\usepackage{dcolumn}
\usepackage{booktabs}							%sch�ne Tabellen
\usepackage{multirow}
\usepackage[normalem]{ulem} %emphasize weiterhin kursiv


%------------------------------------------------------------
% PDF
%------------------------------------------------------------
%\newif\ifpdf
%\ifx\pdfoutput\undefined
%  \pdffalse % we are not running PDFLaTeX
%\else
%  \pdfoutput=1 % we are running PDFLaTeX
%  \pdftrue
%\fi
\usepackage{ifpdf}
\ifpdf
% PDF Settings
\pdfcompresslevel=0
\usepackage{pdflscape}						%wie lscape nur f�r PDF
\usepackage{epstopdf}
%\usepackage[T1]{fontenc}
%\usepackage{ae}                   %nicht mehr n�tig, da mit \usepackage[T1]{fontenc} die cm-super eingebunden werden
%\usepackage[colorlinks=true,breaklinks=false,draft=false,urlcolor=blue,linkcolor=blue,citecolor=black]{hyperref}  %so sp�t wie m�glich laden
%\hypersetup{backref=true,breaklinks=true,urlcolor=blue,pagebackref=true}
\pdfinfo{
%	/Author ()
%	/Title ()
%  %/CreationDate (D:200303272460600)   %Wird automatisch gesetzt
%	/Subject ()
%	/Keywords ()
}
\else
%\usepackage{ae}                   		 %z.B. n�tig, um > in DVI richtig darzustellen
\fi


\newtheorem{thm}{Definition}[section]


%newcommands

\newcommand{\mycomment}[1]{
%#1
}

% eine Randnote fuer fehlende Teile 
\newcommand{\fehlt}[1]{(\marginpar[\hfill!$\longrightarrow$]{$\longleftarrow$!}Hier fehlt \emph{#1})}

% eine Randnote fuer R�ckfrage Teile 
\newcommand{\ccheck}[1]{(\marginpar[\hfill!$\longrightarrow$]{$\longleftarrow$!} \emph{#1})}


%GLEITOBJEKTE
%\renewcommand{\textfraction}{0}    %Legt den Anteil des Platzes einer Seite mit Gleitobjekten fest, der mindestens f�r Text zur Verf�gung steht. Zwischen 0 und 1.
%\renewcommand{\topfraction}{0}    %Legt den Anteil des Platzes am oberen Rand einer Seite fest, bis zu dem Gleitobjekte plaziert werden k�nnen.Zwischen 0 und 1.
%\renewcommand{\bottomfraction}{0}    %Legt den Anteil des Platzes einer Seite fest, den Gleitobjekte (z.B. Abbildungen) am unteren Seitenrand einnehmen k�nnen. Zwischen 0 und 1.
%\renewcommand{\floatpagefraction}{0.9}    %Definiert den Anteil einer Gleitobjekt-Seite, der belegt sein mu�, bevor eine weitere Seite angelegt wird. Zwischen 0 und 1.
%\setcounter{totalnumber}{20}    %Definiert die Anzahl an Gleitobjekten, die h�chstens auf einer Seite angeordnet werden k�nnen. 
